PaCo: Preconditions Attributed to Commonsense Knowledge

Humans can seamlessly reason with circumstantial preconditions of commonsense knowledge. We understand that a glass is used for drinking water, unless the glass is broken or the water is toxic. Despite state-of-the-art (SOTA) language models' (LMs) impressive performance on inferring commonsense knowledge, it is unclear whether they understand the circumstantial preconditions. To address this gap, we propose a novel challenge of reasoning with circumstantial preconditions. We collect a dataset, called PaCo, consisting of 12.4 thousand preconditions of commonsense statements expressed in natural language. Based on this dataset, we create three canonical evaluation tasks and use them to examine the capability of existing LMs to understand situational preconditions. Our results reveal a 10-30% gap between machine and human performance on our tasks, which shows that reasoning with preconditions is an open challenge.

==> Assets/Macros.tex <==
% \renewcommand*{\p@section}{\S\,}
% \renewcommand*{\p@subsection}{\S\,}
% \renewcommand*{\p@subsubsection}{\S\,}

% \definecolor{USCgold}{HTML}{F6C400}
% \definecolor{USCred}{HTML}{990000}

%\newtheorem{mydef}{Definition}

% \theoremstyle{definition}

%####################
\newtheorem{mydef}{Definition}
\newcommand\TODO[1]{\textcolor{red}{#1}}
\newtheorem{definition}{Definition}[section]


%\newcommand{\CS}{commonsense\xspace}
% \newcommand{\CSS}{\CS}

\newcommand{\CN}{ConceptNet\xspace}

\newcommand{\QT}[1]{\emph{#1}\xspace}
% \newcommand{\MCQ}{\QT{requisite}}
\newcommand{\MCQ}{{precondition}\xspace}
\newcommand{\MCQs}{{preconditions}\xspace}
\newcommand{\CQ}{\textit{CoreQuisite}\xspace}
% \newcommand{\CS.}{\CS.}

\newcommand{\muhao}[1]{\textcolor{purple}{[MC: #1]}}
\newcommand{\filip}[1]{\textcolor{blue}{[\textbf{FI:} #1]}}


==> Sections/Motivation.tex <==
One simple way to evaluate any system's understanding is through text completion or question answering.
We hereby give some motivating examples by explicitly asking the SOTA language models about the contextual
information.

As shown in Table~\ref{tab:simple-test}, UnifiedQA~\cite{khashabi2020unifiedqa} is unable to obtain any meaningful response from them.
In addition, neither GPT2~\cite{gpt2}, nor UnifiedQA~\cite{khashabi2020unifiedqa} is able to handle such questions meaningfully. 
In \fact, our study will further reveal that understanding such contextual preconditions is where SOTA language modeling technologies commonly fall short.

\begin{table*}
    \centering
    {\small
    \begin{tabular}{lp{0.50\textwidth}p{0.30\textwidth}}
        \hline \textbf{Model} & \textbf{Input} & \textbf{Output}\\
\hline
        % GPT2& A glass is used for drinking water only if& it is being heated inside. \\
        GPT2                  & A glass is used for drinking water only if, the glass
& is covered in a protective coat or can be removed with cold water. \\
        GPT2                  & A glass is used for drinking water only if, the water
& is acidic, not fresh.                                              \\
        % GPT2& A glass is used for drinking water. what makes this impossible?& Because drinking water in China is
% very expensive ...\\
        UnifiedQA-base        & A net is used for catching fish. What makes this impossible?  (A) You are in water
(B) You are in downtown LA
        & You are in water
        \\
        UnifiedQA-base        & A net is used for catching fish. What makes this impossible?
& A net is used for catching fish.                                   \\
        \hline
    \end{tabular}
    }
    \caption{Test of language model's understanding of preconditions}
    \label{tab:simple-test}
\end{table*}

